A Fast Heuristic for Computing Geodesic Cores in Large Networks

Motivated by the increasing interest in applications of graph geodesic convexity in machine learning and data mining, we present a heuristic for computing the geodesic convex hull of node sets in networks. It generates a set of almost maximal outerplanar spanning subgraphs for the input graph, computes the geodesic closure in each of these graphs, and regards a node as an element of the convex hull if it belongs to the closed sets for at least a user specified number of outerplanar graphs. Our heuristic algorithm runs in time linear in the number of edges of the input graph, i.e., it is faster with one order of magnitude than the standard algorithm computing the closure exactly. Its performance is evaluated empirically by approximating convexity based core-periphery decomposition of networks. Our experimental results with large real-world networks show that for most networks, the proposed heuristic was able to produce close approximations significantly faster than the standard algorithm computing the exact convex hulls. For example, while our algorithm calculated an approximate core-periphery decomposition in 5 hours or less for networks with more than 20 million edges, the standard algorithm did not terminate within 50 days.

==> sections/related_work.tex <==
\section{Related Work}
Several recent works, use geodetic and other closure systems on graphs in the context of graph analysis and node classification. \cite{Sub18} analyse complex networks by considering geodesic subsets. Cunha and Protti \cite{Cunha18} use different closure operators, especially geodesic closure operators in the context of genome rearrangement problems. They show that ... . In \cite{Macedo19} nodes are classified using geodesic closures together with maximization problem expressed by linear integer programming. 
In case of online-learning in graphs Thießen and Gärtner provide an algorithm using geodetic closures. 


==> sections/tables/bigtable.tex <==
\toprule
Graph &       Size &      Edges &  Size Core &  Edges Core & Time [s] exact &  Approx. Core & Time [s] Approx &      Jaccard Similarity (best) \\
\midrule
soc-LiveJournal1 & 4843953.00 & 43,362,750 &        NaN &         NaN &      -1.00e+00 &    3018149.00 &        8.68e+03 &       nan (nan (nan,nan,nan\%)) \\
com-lj.ungraph & 3997962.00 & 34,681,189 &        NaN &         NaN &      -1.00e+00 &    2593060.00 &        1.57e+04 &       nan (nan (nan,nan,nan\%)) \\
soc-pokec-relationships & 1632803.00 & 22,301,964 &        NaN &         NaN &      -1.00e+00 &    1390297.00 &        6.50e+03 &       nan (nan (nan,nan,nan\%)) \\
roadNet-CA & 1957027.00 &  2,760,388 &  328856.00 &   506843.00 &       1.35e+06 &    1102657.00 &        5.16e+03 &   0.23 (0.26 (0.0,10.0,0.05\%)) \\
com-youtube.ungraph & 1134890.00 &  2,987,624 &  390825.00 &  2169158.00 &       8.95e+05 &     296393.00 &        2.88e+03 &   0.73 (0.74 (0.0,10.0,0.01\%)) \\
roadNet-TX & 1351137.00 &  1,879,201 &   39024.00 &    57142.00 &       2.66e+05 &     832817.00 &        3.43e+03 &    0.05 (0.07 (0.0,5.0,0.05\%)) \\
roadNet-PA & 1087562.00 &  1,541,514 &  109968.00 &   162557.00 &       2.59e+05 &     812254.00 &        2.88e+03 &    0.13 (0.16 (0.0,5.0,0.05\%)) \\
Email-EuAll &  224832.00 &    340,795 &   21863.00 &   120633.00 &       8.92e+03 &       5207.00 &        2.58e+02 &  0.24 (0.6 (0.0,1000.0,0.01\%)) \\
Slashdot0902 &   82168.00 &    582,533 &   48718.00 &   514338.00 &       1.39e+04 &      33237.00 &        9.94e+01 &  0.68 (0.8 (0.0,1000.0,0.01\%)) \\
Cit-HepPh &   34401.00 &    420,828 &   32111.00 &   417050.00 &       6.09e+03 &      31443.00 &        5.51e+01 & 0.97 (0.98 (0.0,1000.0,0.01\%)) \\
Cit-HepTh &   27400.00 &    352,059 &   24832.00 &   347918.00 &       3.53e+03 &      24500.00 &        4.54e+01 & 0.98 (0.98 (0.0,1000.0,0.01\%)) \\
Email-Enron &   33696.00 &    180,811 &   10424.00 &   129423.00 &       7.47e+02 &       9595.00 &        4.60e+01 &  0.79 (0.81 (0.0,500.0,0.01\%)) \\
CA-AstroPh &   17903.00 &    197,031 &    9487.00 &   142943.00 &       6.35e+02 &       9680.00 &        2.91e+01 &  0.93 (0.95 (0.0,100.0,0.02\%)) \\
CA-CondMat &   21363.00 &     91,342 &    8603.00 &    49682.00 &       3.95e+02 &       9428.00 &        3.43e+01 &   0.9 (0.94 (0.0,500.0,0.04\%)) \\
CA-HepPh &   11204.00 &    117,649 &    4825.00 &    63548.00 &       1.84e+02 &       5025.00 &        1.76e+01 &  0.91 (0.93 (0.0,100.0,0.03\%)) \\
Wiki-Vote &    7066.00 &    100,736 &    4579.00 &    98026.00 &       1.30e+02 &       3561.00 &        8.68e+00 & 0.78 (0.92 (0.0,1000.0,0.01\%)) \\
facebook-combined &    4039.00 &     88,234 &    2645.00 &    76817.00 &       4.80e+01 &       3112.00 &        6.93e+00 &    0.78 (0.78 (0.0,5.0,0.01\%)) \\
CA-HepTh &    8638.00 &     24,827 &    3605.00 &    14161.00 &       4.60e+01 &       3824.00 &        1.18e+01 &  0.93 (0.96 (0.0,100.0,0.04\%)) \\
CA-GrQc &    4158.00 &     13,428 &    1336.00 &     5036.00 &       7.00e+00 &       1494.00 &        5.73e+00 &  0.88 (0.92 (0.0,100.0,0.05\%)) \\
\bottomrule

==> sections/tables/bigtableold.tex <==
\toprule
Graph &    \multicolumn{1}{c}{Size}   &    \multicolumn{1}{c}{\#Edges}    &  \multicolumn{1}{c}{Density} &  \multicolumn{1}{c}{Size} &   \multicolumn{1}{c}{\#Edges} & \multicolumn{1}{c}{Time [s]} & \multicolumn{1}{c}{Approx.} & \multicolumn{1}{c}{Time [s]} & \multicolumn{1}{c}{Jaccard} \\
&    \multicolumn{1}{c}{$n$}   &    \multicolumn{1}{c}{$m$}    &  \multicolumn{1}{c}{} &  \multicolumn{1}{c}{Core} &   \multicolumn{1}{c}{Core} & \multicolumn{1}{c}{Exact} & \multicolumn{1}{c}{Core} & \multicolumn{1}{c}{Approx.} & \multicolumn{1}{c}{Similarity (best)} \\
\midrule
%			Email-EuAll &   224,832 &     340,795 & 1.30e-05 &  21,863 &   120,633 &       8.92e+03 &       5,469 & 2.35e+02 &       0.25 (0.69 (10000, 1\%))\\
com-amazon.ungraph &   334,863 &     925,872 & 1.70e-05 & 216,109 &   643,075 &       2.20e+05 &   231,285 & 4.73e+02 &       \textbf{0.87} (\textbf{0.88} (500, 3\%))\\
com-dblp.ungraph &   317,080 &   1,049,866 & 2.10e-05 &  90,077 &   438,265 &       7.02e+04 &   100,142 & 4.88e+02 &       \textbf{0.87} (\textbf{0.92} (500, 4\%))\\
web-NotreDame &   325,729 &   1,117,563 & 2.10e-05 &  60,160 &   292,420 &       2.64e+04 &    46,918 & 3.26e+02 &       0.54 (0.59 (100, 1\%))\\
web-Stanford &   255,265 &   1,941,926 & 6.00e-05 &  94,953 & 1,070,885 &       7.98e+04 &       77,534 &      6.35e+02 &        0.36 (0.42 (100, 1\%))\\
Slashdot0902 &    82,168 &     582,533 & 1.73e-04 &  48,718 &   514,338 &       1.39e+04 &    33,405 & 9.18e+01 &       0.68 (0.77 (500, 1\%)) \\
Email-Enron &    33,696 &     180,811 & 3.19e-04 &  10,424 &   129,423 &       7.47e+02 &       9,625 & 4.36e+01 &       \textbf{0.79} (\textbf{0.81} (500, 1\%))\\
CA-CondMat &    21,363 &      91,342 & 4.00e-04 &   8,603 &    49,682 &       3.95e+02 &     9,431 & 3.19e+01 &       \textbf{0.90} (\textbf{0.94} (500, 4\%))\\
CA-HepTh &     8,638 &      24,827 & 6.66e-04 &   3,605 &    14,161 &       4.60e+01 &     3,812 & 1.13e+01 &       \textbf{0.93} (\textbf{0.96} (300, 4\%)) \\
Cit-HepPh &    34,401 &     420,828 & 7.11e-04 &  32,111 &   417,050 &       6.09e+03 &    31,452 & 5.16e+01 &     \textbf{0.97} (\textbf{0.98} (500, 1\%)) \\
Cit-HepTh &    27,400 &     352,059 & 9.38e-04 &  24,832 &   347,918 &       3.53e+03 &    24,504 & 4.19e+01 &       \textbf{0.98} (\textbf{0.98} (400 1\%)) \\
CA-AstroPh &    17,903 &     197,031 & 1.23e-03 &   9,487 &   142,943 &       6.35e+02 &     9,713 & 2.79e+01 &       \textbf{0.93} (\textbf{0.95} (500, 3\%)) \\
CA-GrQc &     4,158 &      13,428 & 1.55e-03 &   1,336 &     5,036 &       7.00e+00 &     1,503 & 5.53e+00 &       \textbf{0.88} (\textbf{0.92} (10, 3\%)) \\
CA-HepPh &    11,204 &     117,649 & 1.87e-03 &   4,825 &    63,548 &       1.84e+02 &     5,022 & 1.70e+01 &       \textbf{0.91} (\textbf{0.93} (100, 3\%))\\
Wiki-Vote &     7,066 &     100,736 & 4.04e-03 &   4,579 &    98,026 &       1.30e+02 &     3,568 & 8.27e+00 &       \textbf{0.78} (\textbf{0.88} (500, 1\%)) \\
facebook\_combined &     4,039 &      88,234 & 1.08e-02 &   2,645 &    76,817 &       4.80e+01 &     3,149 & 6.59e+00 &       \textbf{0.78} (\textbf{0.78} (5, 1\%)) \\
\bottomrule
